Active-Perceptive Motion Generation for Mobile Manipulation

Mobile Manipulation (MoMa) systems incorporate the benefits of mobility and dexterity, due to the enlarged space in which they can move and interact with their environment. However, even when equipped with onboard sensors, e.g., an embodied camera, extracting task-relevant visual information in unstructured and cluttered environments, such as households, remains challenging. In this work, we introduce an active perception pipeline for mobile manipulators to generate motions that are informative toward manipulation tasks, such as grasping in unknown, cluttered scenes. Our proposed approach, ActPerMoMa, generates robot paths in a receding horizon fashion by sampling paths and computing path-wise utilities. These utilities trade-off maximizing the visual Information Gain (IG) for scene reconstruction and the task-oriented objective, e.g., grasp success, by maximizing grasp reachability. We show the efficacy of our method in simulated experiments with a dual-arm TIAGo++ MoMa robot performing mobile grasping in cluttered scenes with obstacles. We empirically analyze the contribution of various utilities and parameters, and compare against representative baselines both with and without active perception objectives. Finally, we demonstrate the transfer of our mobile grasping strategy to the real world, indicating a promising direction for active-perceptive MoMa.

==> 1_related.tex <==
\section{Related Work}
In the context of mobile robots, many active perception methods have been proposed for motion generation using a Next-Best-View (NBV) strategy \cite{Isler16, Watkins21, Naazare22}. (TODO: Add more citations) Typically, the robot's objective is reconstruction, i.e., obtaining complete volumetric information about the scene or target object. Most NBV methods choose a viewpoint based on information gain (IG). The objective is to minimize uncertainty about the scene/object and discover unobserved regions. A good overview and comparison of different IG formulations for NBV is provided in \cite{Delmerico18}.

In the context of grasping, some recent methods have adopted grasp quality metrics to choose the next robot viewpoint that minimizes uncertainty in the grasp pose estimate \cite{Morrison19, Breyer22}. The authors of \cite{Breyer22}, who base their work on \cite{Isler16, Delmerico18}, exploit the fact that only negligible performance differences can be detected in the different formulations of IG computed on an incomplete volumetric representation. They choose the rear side voxel IG formulation and compute IG per proposed next view, equally distributed on a half-sphere above the object, via ray-casting. The active perception is considered complete when a stable grasp quality has been perceived. 

While such active grasping approaches show promise for static manipulation/grasping tasks, there are several drawbacks when considering their application toward mobile manipulation. Firstly, for mobile manipulators, the overall viewing trajectory is important since visual information is gathered over whole trajectories, and we wish to avoid wasteful movement of the whole robot. Secondly, unlike static manipulator scenarios, for mobile manipulation, the reachability and feasibility of viewpoints and grasps have to be considered in the formulation. For instance, grasps that have a high likelihood of success but are challenging to reach can again cause large sub-optimal motions of the robot. Towards this end, we propose a motion generation method that considers gains and costs adapted to the mobile manipulation problem. Our pipeline also considers information accumulation and time-efficient task execution in the same formulation, ensuring the robot can smoothly move between exploration and exploitation behaviors.
